Memorization in deep learning: A survey

Deep Learning (DL) powered by Deep Neural Networks (DNNs) has revolutionized various domains, yet understanding the intricacies of DNN decision-making and learning processes remains a significant challenge. Recent investigations have uncovered an interesting memorization phenomenon in which DNNs tend to memorize specific details from examples rather than learning general patterns, affecting model generalization, security, and privacy. This raises critical questions about the nature of generalization in DNNs and their susceptibility to security breaches. In this survey, we present a systematic framework to organize memorization definitions based on the generalization and security/privacy domains and summarize memorization evaluation methods at both the example and model levels. Through a comprehensive literature review, we explore DNN memorization behaviors and their impacts on security and privacy. We also introduce privacy vulnerabilities caused by memorization and the phenomenon of forgetting and explore its connection with memorization. Furthermore, we spotlight various applications leveraging memorization and forgetting mechanisms, including noisy label learning, privacy preservation, and model enhancement. This survey offers the first-in-kind understanding of memorization in DNNs, providing insights into its challenges and opportunities for enhancing AI development while addressing critical ethical concerns.

==> Chapters/background.tex <==
\section{Background}

==> Chapters/bio.tex <==
\vspace{-60pt}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{BioFigure/jiaheng wei.jpg}}]{Jiaheng Wei} is a Ph.D. student from RMIT
University. He received his bachelor's degree and honors bachelor's degree from Deakin University in 2021 and 2022. His research interests include machine learning security and federated learning privacy.
\end{IEEEbiography}

\vspace{-50pt}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{BioFigure/yanjun zhang.jpg}}]{Yanjun Zhang} is currently a Lecturer at the University of Technology Sydney, Australia. She received her PhD degree in computer science from the University of Queensland, in 2021. Her research interests include cybersecurity and privacy, trustworthy machine learning, and software engineering.
\end{IEEEbiography}

\vspace{-50pt}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{BioFigure/leo zhang.jpg}}]{Leo Yu Zhang}(Member, IEEE) is currently a Senior Lecturer, Griffith University, Brisbane, QLD 4215, Australia. He received the bachelor’s and master’s degrees in computational mathematics from Xiangtan University in 2009 and 2012, and the Ph.D. degree from the City University of Hong Kong, in 2016. His research interests include applied cryptography and AI related security.
\end{IEEEbiography}

\vspace{+60pt}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{BioFigure/ming ding.jpg}}]{Ming Ding}(Senior Member, IEEE) received the B.S. and M.S. degrees (with First-Class Hons.) in electronics engineering and the Doctor of Philosophy (Ph.D.) degree in signal and information processing from Shanghai Jiao Tong University, Shanghai, China, in 2004, 2007, and 2011, respectively. From April 2007 to September 2014, he worked with the Sharp Laboratories of China, Shanghai, as a Researcher/Senior Researcher/Principal Researcher. He is currently a Senior Research Scientist with Data61, CSIRO, Sydney, NSW, Australia. He has authored over 140 papers in IEEE journals and conferences, all in recognized venues, and around 20 3GPP standardization contributions, as well as a book Multi-Point Cooperative Communication Systems: Theory and Applications (Springer). He also holds 21 U.S. patents and co-invented another 100+ patents on 4G/5G technologies in CN, JP, KR, and EU. His research interests include information technology, data privacy and security, machine learning, and AI. He received several awards for his research work and professional services. He is currently an Editor of IEEE TRANSACTIONS ON WIRELESS COMMUNICATIONS and IEEE WIRELESS COMMUNICATIONS LETTERS. He has served as a guest editor/co-chair/co-tutor/TPC member for many IEEE top-tier journals/conferences.
\end{IEEEbiography}


\vspace{-30pt}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{BioFigure/chao chen.jpg}}]{Chao Chen}(Member, IEEE) is currently a Senior Lecturer, RMIT University, Australia. He received the Ph.D. degree in computer science from Deakin University, Geelong, VIC, Australia, in 2017. His research interests include network traffic classification, insider threat detection, and machine learning security, such as inference attacks on machine learning (ML) models.
\end{IEEEbiography}

\vspace{-30pt}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{BioFigure/kok-leong ong.jpg}}]{Kok-Leong Ong} is a Professor of Business Analytics in the College of Business \& Law, RMIT University. He received the BASc (Hons) and PhD degrees from the Nanyang Technological University, Singapore, in 2000 and 2004, respectively. He is currently working on a range of analytics projects making data actionable through analytics-2-business translation, automation, and applications.
\end{IEEEbiography}

\vspace{-30pt}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{BioFigure/junzhang.jpg}}]{Jun Zhang}(Senior Member, IEEE) is the co-founder and director with the Cybersecurity Lab, Swinburne University of Technology, Australia. He received the PhD degree in computer science from the University of Wollongong, Australia. His research interests include cybersecurity and applied machine learning. He is the chief investigator of several projects in cybersecurity, funded by the Australian Research Council (ARC). He has published more than 100 research papers in many international journals and
conferences.
\end{IEEEbiography}

\vspace{-30pt}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{BioFigure/yang xiang.jpg}}]{Yang Xiang}(Fellow, IEEE) is currently a full professor and the dean of Digital Research \& Innovation Capability Platform, Swinburne University of Technology, Australia. He received the PhD degree in computer science from Deakin University, Australia. His research interests include cyber security, which covers network and system security, data analytics, distributed systems, and networking. In particular, he is currently leading his team developing active defense systems against large-scale distributed network attacks. He is the chief investigator of several projects in network and system security, funded by the Australian Research Council (ARC). He has published more than 200 research papers in many international journals and conferences. He served as an associate editor of the IEEE Transactions on Computers, the IEEE Transactions on Parallel and Distributed Systems, Security and Communication Networks (Wiley), and an editor of the Journal of Network and Computer Applications. He is the coordinator, Asia for IEEE Computer Society Technical Committee on Distributed Processing (TCDP). He is a fellow of the IEEE.
\end{IEEEbiography}


